Effective sketching methods for value function approximation

High-dimensional representations, such as radial basis function networks or tile coding, are common choices for policy evaluation in reinforcement learning. Learning with such high-dimensional representations, however, can be expensive, particularly for matrix methods, such as least-squares temporal difference learning or quasi-Newton methods that approximate matrix step-sizes. In this work, we explore the utility of sketching for these two classes of algorithms. We highlight issues with sketching the high-dimensional features directly, which can incur significant bias. As a remedy, we demonstrate how to use sketching more sparingly, with only a left-sided sketch, that can still enable significant computational gains and the use of these matrix-based learning algorithms that are less sensitive to parameters. We empirically investigate these algorithms, in four domains with a variety of representations. Our aim is to provide insights into effective use of sketching in practice.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{enumitem}


%%%%%%%% Distribution definitions %%%%%%%%%%%%%%%

\newcommand{\normal}{\mathcal{N}}
\newcommand{\given}{|}

%%%%%%%% Matrix/vector definitions %%%%%%%%%%%%%%%

\newcommand{\inlinevec}[2]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1\\#2\end{smallmatrix}\Bigr]}}
\newcommand{\inlinemat}[4]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1 \ \ #2 \\#3 \ \ #4\\\end{smallmatrix}\Bigr]}}
\newcommand{\mathvec}[2]{\left[\begin{array}{c}#1\\#2\end{array} \right] }

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}
%\newcommand{\makevector}[1]{{\mathbf #1}}
\newcommand{\zerovec}{\vec{0}}
\newcommand{\onevec}{\vec{1}}
\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\eye}{\mathbf{I}}

%%%%%%%% Simple math functions %%%%%%%%%%%%%%%
\newcommand{\inv}{{\raisebox{.2ex}{$\scriptscriptstyle-1$}}}
\newcommand{\invt}{{\raisebox{.2ex}{$\scriptscriptstyle-\top$}}}
\newcommand{\pinv}{{\raisebox{.2ex}{$\scriptstyle\dagger$}}}
\newcommand{\sgrad}{\partial}
\newcommand{\sign}[1]{\mathrm{sign}(#1)}
\newcommand{\posdef}{\succeq}
\newcommand{\e}{{\textrm{e-}}}
\newcommand{\Dom}{{\textrm{Dom}}}
\newcommand{\smallinv}[1]{{#1}^{\scalebox{0.5}[0.5]{\( - 1\)}}}

%%%%%%%% Norm definitions %%%%%%%%%%%%%%%
\newcommand{\frob}[1]{\left\| #1 \right\|_F}
\newcommand{\frobsq}[1]{\left\| #1 \right\|_F^2}
\newcommand{\frobsqtr}[1]{\text{tr}\left(#1'#1\right)}
\newcommand{\sqnorm}[1]{\Big\|  #1 \Big\|_{2}}
\newcommand{\spnorm}[1]{\left\|  #1 \right\|_{sp}}
\newcommand{\tracenorm}[1]{\left\|  #1 \right\|_{tr}}
\newcommand{\twonorm}[1]{\left\|  #1 \right\|_2}
\newcommand{\twoone}[1]{\left\|  #1 \right\|_{2,1}}
\newcommand{\bregman}[3]{D_{#1}(#2 \; || \: #3)}

%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % RR numbers
\newcommand{\RRbar}{\overline{\RR}} % RR numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

% Set of [0, infty]
\newcommand{\RRpos}{{\RR^+}}

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\eigs}{\mathop{\mathrm{eigs}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nulls}{\mathop{\mathrm{null}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\spec}{\mathop{\mathrm{sp}}}
\newcommand{\sspan}{{\textrm{span}}}
\newcommand{\svd}{\mathop{\mathrm{svd}}}
\newcommand{\te}{\mathop{\mathrm{te}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\DeclareMathOperator\arctanh{arctanh}
%\newcommand{\ln}{\mathop{\mathrm{ln}}}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\set}[2]{\{#1 \ | \ #2\}}
\newcommand{\subfigurespace}[1]{ % Reasonable value = 0.1
\begin{minipage}[b]{#1\textwidth}
 \textbf{ }
 \end{minipage}}
 \newcommand{\figspace}{\begin{minipage}[b]{0.1\textwidth} \textbf{ } \end{minipage}}
\newcommand{\unaryminus}{\scalebox{0.75}[1.0]{\( - \)}}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}


%%%%%%%% Text definitions %%%%%%%%%%%%%%%

\newcommand{\apriori}{{\emph{a priori}}}
\newcommand{\emphdef}[1]{\textbf{#1}}
\newcommand{\introword}[1]{\textbf{\emph{#1}}}
\newcommand{\emphstart}[1]{\textbf{#1}}
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\subheader}[1]{
\vspace{8pt}
\noindent
{\large\bfseries #1}}

%%%%%%%% Examples of Stock standard definitions %%%%%%%%%%%%%%%
% This is just here as a reference for naming convention

%\newcommand{\xb}{\mathbf{x}}
%\newcommand{\xbtil}{\tilde{\xb}}
%\newcommand{\xtil}{\tilde{x}}
%\newcommand{\xhat}{\hat{x}}
%\newcommand{\xbhat}{\hat{\xb}}
%\newcommand{\Xtil}{\tilde{X}}
%\newcommand{\xbar}{\bar{x}}
%\newcommand{\xbbar}{\bar{\xb}}
%\newcommand{\Xb}{\mathbf{X}}
%\newcommand{\Xbtil}{\tilde{\Xb}}
%\newcommand{\Xbar}{\bar{X}}
%\newcommand{\Xbbar}{\bar{\Xb}}
%\newcommand{\Xhat}{\hat{X}}
%\newcommand{\Xbhat}{\hat{\Xb}}
%\newcommand{\Xcal}{\mathcal{X}}
%\newcommand{\Xtilde}{\widetilde{X}}
%\newcommand{\xvec}{\vec{x}}
%\newcommand{\Xvec}{\vec{X}}
%\newcommand{\xvecbar}{\bar{\vec{x}}}
%\newcommand{\xvechat}{\hat{\vec{x}}}
%\newcommand{\valhat}{\hat{\val}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\newcommand{\eproof}{$\null\hfill\blacksquare$}
%\ifx\proof\undefined
%\renewenvironment{proof}{\par\noindent{\bf Proof:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\newenvironment{proofsketch}{\par\noindent{\bf Proof Sketch:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
%\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

% If end proof with align, then can add a negative space to bring up proof box
\newcommand{\palignbox}{\par \vspace{-0.8cm}}
\newcommand{\reducealignspace}[1]{\par \vspace{#1}}

\newif\ifsamenumbers

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\ifsamenumbers
\newtheorem{lemma}[theorem]{Lemma}
\else
\newtheorem{lemma}{Lemma}
\fi
\fi

\ifx\proposition\undefined
\ifsamenumbers
\newtheorem{proposition}[theorem]{Proposition}
\else
\newtheorem{proposition}{Proposition}
\fi
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\ifsamenumbers
\newtheorem{corollary}[theorem]{Corollary}
\else
\newtheorem{corollary}{Corollary}
\fi
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\ifsamenumbers
\newtheorem{conjecture}[theorem]{Conjecture}
\else
\newtheorem{conjecture}{Conjecture}
\fi
\fi

\ifx\axiom\undefined
\newtheorem{axiom}{Axiom}
\fi

\ifx\claim\undefined
\ifsamenumbers
\newtheorem{claim}[theorem]{Claim}
\else
\newtheorem{claim}{Claim}
\fi
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\myintertext}[1]{\end{enumerate} #1\begin{enumerate}[resume]}
\newenvironment{cenumerate}{%
\vspace{10pt}
\noindent{\Large\bfseries Contributions:}
\begin{enumerate}[label={\textbf{Contribution \arabic*.}\ },leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
}
{\end{enumerate}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}
\newcommand{\pca}{\text{\sc pca}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}



==> experiments.tex <==

\section{Experiments}

In this section, we demonstrate on two benchmark domains that the two side random projection approach generally does much worse than one side projection. We then further showed that with one-side projection, we are able to incrementally maintain the pseudoinverse of the $\Amat$ as preconditioner matrix, achieving an unbiased solution even with a low projected dimension. We finally use higher dimensional domain to illustrate the practical usability of our sketching approach. Meanwhile, we also show its favorable efficiency comparing with the ATD paper which incrementally maintain an SVD to the preconditioner matrix. Given the similar performances of differen sketching methods, we fixed using Gaussian random projection in all below experiments. Please refer to the appendix for a detailed experimental setting. 

\paragraph{Neccessity of using one-side projection.} In Figure~\ref{fig:compare_skts50r}, we tested four widely used random projection approaches on two benchmark domains: mountain car and puddle world. First, we showed that the different random projection approaches perform very similar to each other. Second, in Figure~\ref{fig:mcar_lc} we compare the gaussian two-side random projection against gaussian one-side random projection, showing that one-side random projection can generally do better. It means that we should sketch the $\Amat$ matrix instead of sketching the representation matrix $\Phimat$ in linear value function approximation problem. We want to emphasize that our one-side projection technique suffers to low parameter sensitivity as shown in Figure Figure~\ref{fig:mcar_lc}, and we fixed the initialization as identity matrix across all experiments.

We highlight that even with a low dimensional random projection, we can achieve unbiased solution when using the sketched matrix as preconditioner and applying regularization technique proposed by \citep{pan2017accelerated}. Figure~\ref{fig:pd_rank_lc} shows how performance of different algorithms change as rank increasing. Further more, with RBF representation, the sketching technique can significantly outperform TD algorithms and their performance is very close to LSTD. We should be aware that the sketching achieves almost linear time complexity, which is much more efficient than the singular value decomposition approach in \cite{pan2017accelerated}. 

\paragraph{Effects of RBF overlap and feature redundancy.} Since we observed that sketching is more beneficial on RBF representation, we further examined the learning performance on it. First, we consider how the performance changes when we increase the RBF width. Figure~\ref{fig:pd_overlap_redund} shows that the performance of those projection methods are closer to LSTD when we increase the width parameter. 


\begin{figure*}[htp!]
	\vspace{-3cm}
	\centering
	\subfigure[Puddle world, RBF, $\rdim = 25$]{
		\includegraphics[width=\figwidththree]{figures/pd_gau_rbf25r.pdf} \label{fig:pd_gau_rbf25r}} 
	\subfigure[Puddle world, RBF, $\rdim = 50$]{
		\includegraphics[width=\figwidththree]{figures/pd_gau_rbf50r.pdf} \label{fig:pd_gau_rbf50r}}
	\subfigure[Puddle world, RBF, $\rdim = 75$]{
		\includegraphics[width=\figwidththree]{figures/pd_gau_rbf75r.pdf}\label{fig:pd_gau_rbf75r}}
	%\begin{minipage}{\figwidththree}
	%	\vspace{-10.0cm}
		\caption{ 
			The three figures show how performance change when projected dimension $\rdim$ increases from $25$ to $75$. The results are averaged over $50$ runs. One can see that though two-side projection improved a lot when increase $\rdim$, left-side projection can still significantly outperform it. As for left-side projected ATD, it can achieve unbiased performance even when $\rdim = 50$, with much less sensitivity than TD.
		}\label{fig:pd_rank_lc}
	%\end{minipage}
	%\vspace{-0.5cm}	
\end{figure*}

\begin{figure*}[htp!]
	%\centering
	\subfigure[RBF, $\rdim = 50$]{
		\includegraphics[width=\figwidththree]{figures/pd_overlap_rbf50r.pdf} \label{fig:pd_dense_tile50r}}
	\subfigure[Spline, $\rdim = 50$]{
		\includegraphics[width=\figwidththree]{figures/pd_overlap_spline50r.pdf} \label{fig:pd_dense_rbf50r}} \\
	\subfigure[Tile coding, $\rdim = 50$]{
		\includegraphics[width=\figwidththree]{figures/pd_redund_tile50r.pdf} \label{fig:pd_tile_redund}}
	\subfigure[Tile coding style RBF, $\rdim = 50$]{
			\includegraphics[width=\figwidththree]{figures/pd_redund_tilerbf50r.pdf} \label{fig:pd_tilerbf_redund}}
	\begin{minipage}{\figwidththree}
	\vspace{-8.0cm}
	\caption{ 
		%\small
		In figure \textbf{(a)} and \textbf{(b)}, we use puddle world domain as an example to explore how the RBF width changes would influence the sketching performance. The x-axis corresponds to four width parameter values: $0.0510, 0.0849, 0.1200, 0.1039$. Figure \textbf{(c)} and \textbf{(d)} show how performance changes when we increase feature redundancy on tile coding and tile-coding-style RBF. For both figures, the three tile coding settings corresponding to the three ticks on x-axis are $4 \times 16 \times 16, 16 \times 8 \times 8, 64 \times 4 \times 4$. A rough conclusion from these figures is: random projection sketching prefers a relatively dense representation, since their performance is closer to LSTD as density increases. 
	}\label{fig:pd_overlap_redund}
 \end{minipage}
	%\vspace{-0.5cm}	
\end{figure*}

\paragraph{Experiments on high dimensional domains.} We now apply our sketching techniques on two high dimensional domain to illustrate practical usability: acrobot and energy allocation. The acrobot domain, as described in \cite{sutton1998reinforcement}, is a four dimensional episodic task domain which we convert to $2^{15} = 32,768$ binary features under tile coding. The task is to raise the arm to a certain level. As for the energy allocation domain, we use exact same tile coding setting from ATD paper \cite{pan2017accelerated}, where $8192$ tile coding features are generated. 

\begin{figure*}[htp!]
	\centering
	\subfigure[Acrobot domain, RBF]{
		\includegraphics[width=\figwidththree]{figures/acro_gau_rbf50r.pdf}\label{fig:acro_rbf50r}}	
	\subfigure[Acrobot domain, RMSE vs Time]{
		\includegraphics[width=\figwidththree]{figures/acro_time_50r.pdf}}
	\subfigure[Energy allocation, Tile coding]{
		\includegraphics[width=\figwidththree]{figures/energy_gau_tile50r.pdf}\label{fig:energy_tile50r}}
	%\vspace{-5.0cm}
	\caption{ 
		%\small
		Both figures are using projected dimension $\rdim = 50$, results are averaged over $30$ runs. We see that sketching can converge faster than TD algorithms. And the sketching method is highly efficient, performs best in figure \textbf{(b)} when we restrict number of samples to $25$ per second. Energy domain is optimized over the last half of steps to avoid blowing up at the tail for TD algorithms. On this domain, the two-side projection method (LSTD-P, ATD-P) is significantly worse than other algorithms. 
		\\
	}\label{fig:high_domain}
	%\vspace{-0.5cm}	
\end{figure*}

